Wonder3D: Single Image to 3D using Cross-Domain Diffusion

In this work, we introduce Wonder3D, a novel method for efficiently generating high-fidelity textured meshes from single-view images.Recent methods based on Score Distillation Sampling (SDS) have shown the potential to recover 3D geometry from 2D diffusion priors, but they typically suffer from time-consuming per-shape optimization and inconsistent geometry. In contrast, certain works directly produce 3D information via fast network inferences, but their results are often of low quality and lack geometric details. To holistically improve the quality, consistency, and efficiency of image-to-3D tasks, we propose a cross-domain diffusion model that generates multi-view normal maps and the corresponding color images. To ensure consistency, we employ a multi-view cross-domain attention mechanism that facilitates information exchange across views and modalities. Lastly, we introduce a geometry-aware normal fusion algorithm that extracts high-quality surfaces from the multi-view 2D representations. Our extensive evaluations demonstrate that our method achieves high-quality reconstruction results, robust generalization, and reasonably good efficiency compared to prior works.

==> figures/ablation-normal-benfit.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_ablation-normal-benefit.pdf}
\caption{The effect of learning the normal domain to the color domain. Compared to the single color diffusion model, the cross-domain diffusion model can improve the quality of the generated multi-view color images. \LC{The first row does not show significant improvement, it would be good to change an example.}}
%红框
\label{fig:ablation_normal_benefit}	
\end{figure}

==> figures/cross-domain.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/fig_cross-domain.pdf}
\caption{}
%红框
\label{ablation_cross_domain}	
\end{figure}
